Transfer Learning from Simulated to Real Scenes for Monocular 3D Object Detection

Accurately detecting 3D objects from monocular images in dynamic roadside scenarios remains a challenging problem due to varying camera perspectives and unpredictable scene conditions. This paper introduces a two-stage training strategy to address these challenges. Our approach initially trains a model on the large-scale synthetic dataset, RoadSense3D, which offers a diverse range of scenarios for robust feature learning. Subsequently, we fine-tune the model on a combination of real-world datasets to enhance its adaptability to practical conditions. Experimental results of the Cube R-CNN model on challenging public benchmarks show a remarkable improvement in detection performance, with a mean average precision rising from 0.26 to 12.76 on the TUM Traffic A9 Highway dataset and from 2.09 to 6.60 on the DAIR-V2X-I dataset when performing transfer learning. Code, data, and qualitative video results are available on the project website: https://roadsense3d.github.io.

==> notes.tex <==
% ---------------------------------------------------------------
% OPENREVIEW profiles:
% ---------------------------------------------------------------
% https://openreview.net/profile?id=~Sondos_Mohamed1 (s.mohamed@studenti.unica.it)
% https://openreview.net/profile?id=~Walter_Zimmer1 (walter.zimmer@tum.de)
% https://openreview.net/profile?id=~Ross_Greer1 (rossgreer@ucmerced.edu)
% https://openreview.net/profile?id=~Ahmed_Alaaeldin_Ghita1 (ahmed.ghita@setlabs.de)
% https://openreview.net/profile?id=~Mirko_Marras1 (mirko.marras@unica.it, supervisor of Sondos)
% https://openreview.net/profile?id=~Mohan_Trivedi1 (mtrivedi@ucsd.edu)
% https://openreview.net/profile?id=~Alois_Knoll1 (k@tum.de)


% ---------------------------------------------------------------
% DONE: 12 TASKS COMPLETED :)
% ---------------------------------------------------------------
% [x] Sondos: describe how Cube R-CNN was selected -> mention selection criteria
% [x] Walter: update title
% [x] Walter: Revise related work 
% [x] Walter: Update tables with related datasets and models
% [x] W: Improve the related work architecture (integrity, coherence).
% [x] W: Revise the references (especially Table 1 and Table 2).
% [x] S: Add section criteria for the models and dataset (based on the discussion during the meeting).
% [x] S: Provide a brief explanation of the selected models (5 selected models).
% [x] S: Apply additional filters (to select Cube R-CNN).
% [x] Sondos: Describe the RoadSense3D++ synthetic dataset. How many frames are labeled? Under what lighting and weather conditions? How many objects are annotated? How are they distributed?
% [x] Ahmed: finish conclusion section. Write the conclusion (Ahmed will wait for Sondos to add the final result for DairxV2X).
% [x] S: EXPERIMENT 1: train on A9 dataset from scratch and evaluate on A9. Create qualitative results (visualize 3D detections and labels on A9 test images). Pretrain on RoadSense, then fine-tune on A9 dataset, then evaluate again on A9 and you should get better/higher results. Create qualitative results (visualize 3D detections after fine-tuning with 3D labels on the same A9 test images)
% ---------------------------------------------------------------

% ---------------------------------------------------------------
% TODOS FOR CAMERA-READY VERSION : Sorted by priority
% ---------------------------------------------------------------
% [x] S: EXPERIMENT 2: train on DAIR-V2X dataset from scratch and evaluate on DAIR-V2X. Create qualitative results (visualize 3D detections and labels on DAIR-V2X test images). Pretrain on RoadSense, then fine-tune on DAIR-V2X dataset, then evaluate again on DAIR-V2X and you should get better/higher results. Create qualitative results (visualize 3D detections after fine-tuning with 3D labels on the same DAIR-V2X test images)
% [] S: EXPERIMENT 3: use the pretrained model from EXPERIMENT 2 (pretrained on RoadSense and DAIR-V2X) and fine-tune it on A9. Then evaluate it on A9 dataset and you should get higher results than in the  first experiment :) Create qualitative results (visualize 3D detections and labels on A9 test images after fine-tuning on A9). Create qualitative results (visualize 3D detections and labels on A9 test images after fine-tuning on A9). To show the effect of transfer learning from large to small dataset. Pretrain on DAIR-V2X only, then fine-tune on A9.
% [] Sondos: To minimize the sim-to-real gap you should normalzie the vehicle dimensions of the source dataset to the vehicle dimensions of the target dataset. Proposed by:
%    https://openaccess.thecvf.com/content_CVPR_2020/papers/Wang_Train_in_Germany_Test_in_the_USA_Making_3D_Object_CVPR_2020_paper.pdf
% [x] Sondos: add qualitative results
% [] Sondos: add a short section where you describe the custom real-world dataset (labeled with 3D BAT) -> the number of labels can be also extended after the submission 
% [] S: add transfer learning architecture (flow diagram) on 2. page: (input > 1. dataset > 2. dataset > output)
% [X] Ross: revise the Introduction section, and update contribution
% [] Ross: proof read whole paper and check for English grammar -> you are nativev American English speaker :)
% [] Ahmed: add section about data labeling (process) and 3D BAT annotation tool
% [x] S: add conference/journal to Table 1
% [] S: mention what techniques do you apply to reduce the sim-to-real gap
% [] S: Add figures and more statistics for the simulated datasets.
% [] Sondos: Describe how transfer learning is performed in detail -> methodology
% [] Sondos: add ablation studies (freeze different number of layers)
% [x] R: Revise the integrity and coherence of the introduction.
% [x] R + A: Review the abstract together.
% [] S: add title figure on first page
% [?] W: Revise the title  for the methodology with Sondos (only the caption, because I forgot it).  QUESTION: What do you mean by caption?
% ---------------------------------------------------------------
% [x] add acknowledgement for camera-ready version, for double blind submission: commented
% [] cite 3d object detection paper
